A unified field theory from a complexified quaternion-octonion Dirac equation

It is set manifest an underlying algebraic structure of Dirac equation and solutions, in terms of Cl2 Clifford algebra projectors and ladder operators. From it, a scheme is proposed for constructing unified field theories by enlarging the pointed algebra. A toy unified matter field model is formulated, modifying Dirac equation with complex quaternions and octonions. The result describes a set of fermion fields with reminiscent properties of one standard model particle generation, exhibiting U(1) electromagnetism, SU(2) flavor and SU(3) color like symmetries, remarkably SU(2) induces frame fields, though further explorations are needed.

==> titlepage.tex <==
\thispagestyle{empty}
\begin{center}
\begin{large}
\begin{figure}
    \centering
    \includegraphics[width=3cm]{UVlogo.jpg}
\end{figure}
\noindent\hrulefill 
\\
\vspace{0.5cm}
\begin{Huge}
    \textbf{Heat transport in scanning tunneling spectroscopy with superconductors for spin polarized molecule}
\end{Huge}
\\
\vspace{0.2cm}
\noindent\hrulefill 
\vspace{0.5cm}
\\
by
\\
\vspace{0.5cm}
\textbf{Juan Camilo V\'elez Qui\~nones\vspace{1cm}\\
Supervisor: PhD Juan David Vasquez Jaramillo}
\end{large}\\
\begin{small}
Universidad de Pamplona Facultad de F\'isica y Geolog\'ia Pamplona, Colombia\\
\end{small}
\vspace{0.2cm}
\begin{large}
\textbf{Co-Supervisor: PhD Karen Rodr\'iguez Ram\'irez}\\
\end{large}
\begin{small}
Universidad de Valle, Departamento de F\'isica Cali, Colombia
\end{small}
\vspace{2cm}
\\
\begin{large}
\textit{A Master project submitted as requirement for the Physicist Master program}
\vspace{2cm}
\\
\end{large}
Departamento de F\'isica\\
Facultad de Ciencias Naturales y Exactas\\
Universidad del Valle\\Santiago de Cali, Colombia
\end{center}
